Reducing Protocol Analysis with XOR to the XOR-free Case in the Horn Theory Based Approach

In the Horn theory based approach for cryptographic protocol analysis, cryptographic protocols and (Dolev-Yao) intruders are modeled by Horn theories and security analysis boils down to solving the derivation problem for Horn theories. This approach and the tools based on this approach, including ProVerif, have been very successful in the automatic analysis of cryptographic protocols w.r.t. an unbounded number of sessions. However, dealing with the algebraic properties of operators such as the exclusive OR (XOR) has been problematic. In particular, ProVerif cannot deal with XOR. In this paper, we show how to reduce the derivation problem for Horn theories with XOR to the XOR-free case. Our reduction works for an expressive class of Horn theories. A large class of intruder capabilities and protocols that employ the XOR operator can be modeled by these theories. Our reduction allows us to carry out protocol analysis by tools, such as ProVerif, that cannot deal with XOR, but are very efficient in the XOR-free case. We implemented our reduction and, in combination with ProVerif, applied it in the automatic analysis of several protocols that use the XOR operator. In one case, we found a new attack.

==> back.tex <==
\section{Conclusion}\label{sec:conclusion}

Diffie Hellman

alternative, proverif with unification modulo xor


[\ldots]



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "xorpro"
%%% End: 


==> intruder-rules.tex <==
    \begin{figure}
        \begin{align*} 
            \I(x) &\ra \I(\hash(x)) 
                & \I(x), \I(y) &\ra \I(\an{x,y}) \\[1ex]
            \I(\an{x,y}) &\ra \I(x) 
                & \I(\an{x,y}) &\ra \I(y)\\[1ex]
            \I(x), \I(k) &\ra \I(\senc xk), 
                & \I(\senc xk), \I(k) &\ra \I(x) \\[1ex]
            \I(x), \I(\pub k) &\ra \I(\penc x{\pub k}), 
                & \I(\penc x{\pub k}), \I(k) &\ra \I(x) 
        \end{align*}
        \caption{Intruder Rules.\label{intruder-rules}}
    \end{figure}


==> x-experiments.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation and Experiments}\label{sec:implementationandexperiments}

We have implemented our reduction, and together with
ProVerif, tested it on a set of protocols which employ the
XOR operator. In this section, we report on our
implementation and the experimental results.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation}\label{sec:implementation}

We have implemented our reduction function in SWI prolog
(version 5.6.14).  Our implementation essentially takes a
Horn theory as input. More precisely, the input consists of
(1) a declaration of all the functor symbols used in the
protocol and by the intruder, (2) the initial intruder
facts as well as the protocol and intruder rules, except
for the $\xor$-rule, which is assumed implicitly, (3) a
statement which defines a secrecy or authentication goal.
Moreover, options that are handed over to ProVerif may be
added.


Our implementation then first checks whether the given Horn
theory, say $T$, (part (2) of the input) is $\xor$-linear.
If it is not, an error message is returned. If it is, a set
$\C$ is computed such that the Horn theory is
$\C$-dominated. Recall that such a set always exists if the
Horn theory is $\xor$-linear. It is important to keep $\C$
as small as possible, in order for the reduction to be more
efficient. Once $\C$ is computed, the reduction
function as described in Section~\ref{sec:reduction} is
applied to $T$, i.e., $T^+$ is computed. Now, $T^+$
together with the rest of the original input is passed on
to ProVerif. This tool then does the rest of the work,
i.e., it checks the goals for $T^+$. This is possible
since, due the reduction, the XOR operator in $T^+$ can now
be considered to be an operator without any algebraic
properties.

Our implementation does not follow the construction of the
reduction function described in Section~\ref{sec:reduction}
precisely, in order to produce an output that is optimized
for ProVerif (but still equivalent): a) While terms of the
form $c\xor t$, with $c\in \CC$, $t\notin \CC$ are 
represented by $\tt xor(c,t)$, terms $a\xor b\in \CCnorm$
are represented by $\tt xx(a,b)$. This representation
prevents some unnecessary unifications between terms.
However, it is easy to see that with this representation,
the proofs of soundness and completeness of our reduction
still go through. The basic reason is that terms in
$\CCnorm$ can be seen as constants. b) For the Horn clauses
in Figure~\ref{fig:Tplus},
\eqref{rule:const}--\eqref{rule:gen}, we do not produce
copies for every choice of $c,c'\in \CCnorm$. Instead, we
use a more compact representation by introducing auxiliary
predicate symbols. For example, the family of Horn clauses
in \eqref{rule:variant} is represented as follows:
$\tt{xtab}(x,y,z), I(y), I(\tt{xor}(x,t)) \rightarrow
I(\tt{xor}(z,t))$, where the facts
$\tt{xtab}(c,c',\rep{c\xor c'})$ for every $c,c'\in
\CCnorm$ are added to the Horn theory given to ProVerif.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiments}\label{sec:experiments}

\begin{figure}[!t]
    \centering
    \begin{tabular}{lcrr}
        \sf\footnotesize protocol & \sf\footnotesize correct & \sf\footnotesize reduction time & \sf\footnotesize ProVerif time \\
        \hline\\[-1.2ex]
        \sf NSL$_{\xor}$        & no  & 0.02s & 0.006s \\
        \sf NSL$_{\xor}$-fix    & yes & 0.04s & 0.09s \\
        \sf NSL$_{\xor}$-auth-A & no  & 0.03s & 0.16s \\
        \sf NSL$_{\xor}$-auth-A-fix & yes  & 0.03s & 0.02s \\
        \sf NSL$_{\xor}$-auth-B & yes  & 0.04s & 0.5s \\
        \sf SK3     & yes & 0.05s & 0.3s \\
        \sf RA      & no  & 0.05s & 0.17s \\
        \sf RA-fix  & yes & 0.05s & 0.27s \\
        \sf CCA-0    & no & 1.1s & 109s \\
        \sf CCA-1A        & yes & 0.25s & 0.7s \\
        \sf CCA-1B        & yes & 0.25s & 1.3s \\
        \sf CCA-2B        & yes & 1.1s & 7.1s \\
        \sf CCA-2C        & yes & 1.1s & 58.0s \\
        \sf CCA-2E        & yes & 0.25s & 1.42s 
    \end{tabular}
    \caption{Experimental Results. \label{fig:exp}} 
\end{figure}


We applied our method to a set of ($\xor$-linear)
protocols. The results, obtained by running our
implementation on a 2,4 Ghz Intel CoreTM 2 Duo E6700
processor with 2GB RAM, are depicted in
Figure~\ref{fig:exp}, where we list both the time of the
reduction and the time ProVerif needed for the analysis of
the output of the reduction. We note that except for
certain versions of the CCA protocol, the other protocols
listed in Figure~\ref{fig:exp} are out of the scope of the
implementation in \cite{CortierKeighrenSteel-TACAS-2007},
the only other implementation that we know of for
cryptographic protocol analysis w.r.t.~an unbounded number
of sessions that takes XOR into account. As mentioned in
the introduction, the method in
\cite{CortierKeighrenSteel-TACAS-2007} is especially
tailored to the CCA protocol. It can only deal with
symmetric encryption and the XOR operator, but, for
example, cannot deal with protocols that use public-key
encryption or pairing. Let us discuss the protocols and
settings that we analyzed in more detail.

By \mbox{NSL$_{\xor}$} we denote our running example. Since
there is an attack on this protocol, we also propose a fix
\mbox{\sf NSL$_{\xor}$-fix} in which the message
$\penc{\an{M, N\xor B}}{\pub{sk_A}}$ is replaced by
$\penc{\an{M, h(\an{N,M})\xor B}}{\pub{sk_A}}$ for a hash
function $h(\cdot)$. We analyze both authentication and
secrecy properties for these ($\xor$-linear) protocols.

The ($\xor$-linear) protocol {\sf SK3}
\cite{ShoupRubin-EUROCRYPT-1996} is a key distribution
protocol for smart cards, which uses the XOR operator. {\sf
  RA} denotes an ($\xor$-linear) group protocol for key
distribution \cite{BullOtway-TR-DRA-1997}. Since there is a
known attack on this protocol, we proposed a fix: a message
$k_{A,B} \xor h(\an{\mathsf{key}(A),N})$ sent by the key
distribution server to $A$ is replaced by $k_{A,B}\xor
h(\an{\mathsf{key}(A),\an{N,B}})$.


\begin{figure*}[!t]
%        \def\kp#1{\mathit{k#1}}
         \begin{align}
            I(x),\ I(\e{k}{\km\xor\data})  \rra  
                I(\e{x}{k}) \tag{{\it Encipher}} \label{cca:enc}\\[1ex]
            I(\e x k),\ I(\e k{\km\xor\data} )
                \rra I(x)  \tag{{\it Decipher}} \label{cca:dec} \\[1ex]
            I(\e{k}{\km\xor\typ}),\ I(\typ),\ I(\e{\kek}{\km\xor\exp})
                \rra I(\e{k}{\kek\xor\typ})  \tag{{\it KeyExport}} \label{cca:exp} \\[1ex]
            I(\e{k}{\kek \xor \typ}),\ I(\typ),\ I(\e{\kek}{\km\xor\imp})
                \rra I(\e{k}{\km\xor\typ})  \tag{{\it KeyImport}} \label{cca:imp} \\[1ex]
            I(k1), I(\typ) \rra I(\e{k1}{\km\xor\kp\xor\typ})
                \tag{{\it KeyPartImp-First}} \label{cca:first} \\[1ex]
            I(k2), I(\e{x}{\km\xor\kp\xor\typ}), I(\typ)
                \rra I(\e{x\xor k2}{\km\xor\kp\xor\typ})
                \tag{{\it KeyPartImp-Middle}} \label{cca:middle} \\[1ex]
            I(k3), I(\e{y}{\km\xor\kp\xor\typ}), I(\typ)
                \rra I(\e{y\xor k3}{\km\xor\typ})
                \tag{{\it KeyPartImp-Last}} \label{cca:last} \\[1ex]
            I(\e{k}{\kek_1\xor\typ}),\ I(\typ),\ I(\e{kek_1}{\km\xor\imp}),\
                I(\e{kek_2}{\km\xor\exp})  \rra  I(\e{k}{kek_2\xor\typ})
                \tag{{\it KeyTranslate}} \label{cca:transl}
            % I(\typ) \rra I(\e{\new}{\km\xor\typ}) \tag{{\it Key-Generate}} \label{cca:gen}
         \end{align}
        \caption{CCA API \label{fig:cca}, where $\km$ denotes a constant
          (the key master stored in the cryptographic coprocessor),
          $\typ$ is a constant that ranges over the constants in
          $\{\data,\imp,\exp,\pin\}$, 
          %$\new$ is a constant that stands for a new key, 
          and all other symbols
          ($x$, $y$, $k$, ...) are variables.} 
\end{figure*}

%\subsection{Experiments with CCA}\label{sec:cca-experiments}

{\sf CCA} stands for Common Cryptographic Architecture
(CCA) API \cite{IBM-CCA} as implemented on the hardware
security module IBM 4758 (an IBM cryptographic
coprocessor). The CCA API is used in ATMs and mainframe
computers of many banks to carry out PIN verification
requests. It accepts a set of commands, which can be seen
as receive-send-actions, and hence, as cryptographic
protocols. The only key stored in the security module is
the master key $\km$. All other keys are kept outside of
the module in the form $\e{k}{\km\xor \typ}$, where
$\typ\in \{\data,\imp,\exp,\pin\}$ denotes the type of the
key, where each type is some fixed constant.  The commands
of the CCA API include the following: Commands for
encrypting/decrypting data using data keys. Commands to
export/import a key to/from another security module. This
is done by encrypting/decrypting the key by a
key-encryption-key. 

In Figure~\ref{fig:cca}, we model the most important
commands of the CCA API (see also
\cite{CortierKeighrenSteel-TACAS-2007}) in terms of Horn
clauses.  \eqref{cca:enc} and \eqref{cca:dec} are used to
encrypt/decrypt data by data keys.  \eqref{cca:exp} is used
to export a key to another security module by encrypting it
under a key-encryption-key, with \eqref{cca:imp} being the
corresponding import command. The problem is to make the
same key-encryption-key available in different security
modules. This is done by a secret sharing scheme using the
commands \eqref{cca:first}--\eqref{cca:last}, where $\kp$
is a type (a constant) which stands for ``key part'',
$\kek$ is obtained as $k1\xor k2 \xor k3$, and each $ki$,
$i\in \{1,2,3,\}$, is supposed to be known by only one
individual.  \eqref{cca:transl} is used to encrypt a key
under a different key-encryption-key.

% Finally, with \eqref{cca:gen} new keys can be generated.

We note that some of the Horn clauses in Figure~\ref{fig:cca}, namely
\eqref{cca:middle} and \eqref{cca:last}, are not linear.
Fortunately, one can apply a standard unfolding technique for Horn
clauses together with straightforward simplifications to obtain an
\emph{equivalent} Horn theory with only $\xor$-linear rules.

There are several known attacks on the CCA API, which
concern the key-part-import process. One attack is by Bond
\cite{Bond-CHES-2001}. As a result of this attack the intruder is able
to obtain PINs for each account number by performing
data encryption on the security module. A stronger attack
was found by IBM and is presented in \cite{Clulow-Msc}
where the intruder can obtain a PIN derivation key, and
hence, can obtain PINs even without interacting with the
security module. However, the IBM attack depends on key
conjuring \cite{CortierKeighrenSteel-TACAS-2007}, and
hence, is harder to carry out. Using our implementation
(together with ProVerif) and the configuration denoted by
{\sf CCA-0} in Figure~\ref{fig:exp}, we found a new attack
which achieves the same as the IBM attack, but is more
efficient as it does not depend on key conjuring. Our attack is
presented at the end of this section.

In response to the attacks reported in \cite{Bond-CHES-2001}, IBM
proposed two recommendations.

\medskip

\noindent\emph{Recommendation 1.}  As mentioned, the
attacks exploit problems in the key-part-import process. To
prevent these problems, one IBM recommendation is to
replace this part by a public-key setting. However, as
shown in \cite{CortierKeighrenSteel-TACAS-2007}, further
access control mechanisms are needed, which essentially
restrict the kind of commands certain roles may perform.
Two cases, which correspond to two different roles, are
considered, and are denoted {\sf CCA-1A} and {\sf CCA-1B}
in Figure~\ref{fig:exp}. We note that the Horn theories
that correspond to these cases are $\xor$-linear, and
hence, our tool can be applied directly, no changes are
necessary; not even the transformations mentioned above.
Since public-key encryption (and pairing) cannot be
directly handled by the tool presented by Cortier et
al.~\cite{CortierKeighrenSteel-TACAS-2007}, Cortier et
al.~had to modify the protocol in an ad hoc way, which is
not guaranteed to yield an equivalent protocol. This is
also why the runtimes of the tools cannot be compared
directly.

\medskip

\noindent\emph{Recommendation 2.} 
Here additional access control mechanisms are assumed which
ensure that no single role is able to mount an attack.  We
analyzed exactly the same subsets of commands as the ones
in \cite{CortierKeighrenSteel-TACAS-2007}. These cases are
denoted {\sf CCA-2B}, {\sf -2C}, and {\sf -2E} in
Figure~\ref{fig:exp}, following the notation in
\cite{CortierKeighrenSteel-TACAS-2007}. The runtimes
obtained in \cite{CortierKeighrenSteel-TACAS-2007} are
comparable to ours: 333s for {\sf CCA-2B}, 58s for {\sf
  -2C}, and 0.03s for {\sf -2E}.
    

% \rk{Computer?}

%     We applied our method for a number of protocols that employ the
%     XOR operator. First, we experimented with the variant of
%     Needham-Shroeder protocol from
%     \cite{ChevalierKuestersRusinowitchTuruani-LICS-2003}, SK3 Protocol
%     (Symmetric key distribution using Smart Cards, by Shoup and
%     Rubin), and Recursive Authentication Protocol employing $\xor$
%     (this variant was the original one). These protocols are
%     $\xor$-linear and our method can be applied directly and quite
%     easily to them. 

%     In the next section we describe the experiments with CCS API,
%     which is not $\xor$-linear and so our approach cannot be used
%     directly (to analyze this protocol, we had first to make some
%     transformations by hand). 
    

%     We made experiments with the following protocols which are are
%     $\xor$-linear, provided the number of participants is finite (as
%     we mentioned, for proving secrecy, it is enought to consider only
%     two participants: one honest and one dishonest). In
%     Figure~\ref{fig:exp} results of experiments for the following
%     progocols are presented:
    
%     \begin{enumerate}[(a)]
%      \item
%          A variant of Needham-Shroeder-Lowe protocol from
%          \cite{ChevalierKuestersRusinowitchTuruani-LICS-2003}
%          described in the previous section ({\sf NSL}). This variant
%          is known to be faulty. That is why we propose a version of
%          this protocol with a fix which prevents the attack ({\sf
%          NSL-fix}). It this version we replace the message
%          $\penc{\an{M, N\xor B}}{\pub{sk_A}}$ sent by $B$ to $A$ in
%          step (2) by the message $\penc{\an{M, h(N,M)\xor
%          B}}{\pub{sk_A}}$.

%          Authentication properties for these protocols were also
%          alalysed: {NSL-auth-A} and {\sf NSL-auth-A-fix} correspond
%          to the case when $A$ authenticates to $B$. In the case when
%          $B$ authenticates to $A$, the property can be proven also for
%          the original version.

%      \item
%          \emph{SK3 Protocol} \cite{ShoupRubin-EUROCRYPT-1996} ---
%          symmetric key distribution using Smart Cards, by Shoup and
%          Rubin.

%      \item
%         \emph{Recursive Authentication Protocol} ({\sf RA}) [?] ---
%         It is a quite complex group protocols with a kind of recursive
%         computations. We model these computations using horn clauses
%         in a safe way, i.e.~in a way that preserve secrecy (the
%         modeling resembles the one from
%         \cite{KuestersTruderung-STACS-2007}).  The protocol is known
%         to be faulty, thus we considered also a  version with some fix
%         that prevents attacks ({\sf RA-fix}).  In this version, 
%         a freshly generated session key $k_{A,B}$
%         intended to further communication of $A$ and $B$ is sent 
%         by the server to $A$ in the form
%         $k_{A,B}+h(\mathsf{key}(A),\an{N,B})$ instead of
%         $k_{A,B}+h(\mathsf{key}(A),N)$ as it is done in the original
%         version, where $\mathsf{key}(A)$ is the shared by $A$ and the
%         server, and $N$ is a nonce generated previously by $A$.
%     \end{enumerate}
    
% \section{Analyzing CCA}

%     IBM's Common Cryptographic Architecture (CCA) \cite{IBM-CCA} is
%     an API used by hardware security modules in ATMs and in the
%     mainframe computers of many banks. A hardware security module is
%     essentially a cryptographic coprocessor encased in a tamper-proof
%     enclosure.  The CCA is provided by IBM's 4758 Cryptographic
%     Coprocessor whose main task of the API is to carry out PIN
%     verification requests. 

%     The API can be thought as a set of two party security protocols,
%     which enables us to use the techniques developed for formal
%     verification of security protocols.

%     In 2001, first flaws in the CCA were discovered
%     \cite{Bond-CHES-2001}, and more
%     flaws was discovered since then (for instance an attack found by
%     IBM, described in \cite{Clulow-Msc}). These flaws exploit
%     algebraic properties of $\xor$ operation which is used in the
%     protocol. In response, IBM made changes in version 2.41 of the API
%     and provided several procedural recommendations to prevent the
%     attack. These recommendations, roughly speaking, prevent one
%     single individual from having access to all the commands required
%     to carrying out the attack, which is done by assigning roles to
%     these individuals and by using Access Control System. Each
%     such a role can be seen as a subset of commands and to prove that
%     the whole API is safe, one has to prove it for a number of cases
%     which corresponds to different recommendations and different roles.

%     The API and the recommendations were analyzed in [....], where it
%     is shown that API is secure, if the recommendations are followed.
%     We also apply our method to reprove these results.
%     Unfortunately,  for some cases, the resulting subset of command
%     is not $\xor$-linear, and so our tool cannot be applied directly.
%     However, we managed to verify these cases too, doing some rather
%     simple and well established transformations (which gave an
%     equivalent, $\xor$-linear protocols) on the set of Horn clauses
%     that represents the Intruder knowledge. We stress here that
%     the transformation we did are not on the protocol level, but
%     are applied to the set of Horn clauses, and can be easily proved
%     to produce an result of the same semantics. 

%     Considering the fact that the decidability result presented in [?]
%     works for quite particular family of protocols (without pairing,
%     hashing, public-key encryption, and for very limited usage of
%     symmetric encryption), and the tool described in [?] is a very
%     particular implementation working exclusively with CCA (the CCA
%     rules are directly encode in C), our experiments show that our
%     method is quite general and efficient tool for analyzing
%     protocols with $\xor$ operation. We also note that the method
%     used in [?] do not handle pairing an public key encryption which
%     are used in recommendation 1 described below. Hence, in [?], to handle
%     this recommendation, some changes in the protocol had to be made.
%     With our approach, the cases for recommendation 1 can be precisely
%     modeled.

%     Our tool discovered also a new attack on the API. This attack (like the
%     previously known ones) is possible when recommendations are not
%     followed strictly or when some persons cooperate in order to mount
%     an attack. The attack is described in Section \ref{sect:attack}.

%     \medskip  In the remainder of this section we first describe the
%     CAA API in more detailes and some known attacks. Then we present
%     the recommendations issued by IBM intended to prevent the attacks
%     and we briefly the results discuss our experiments with proving
%     secrecy for these recommendations. Finally, we described an attack
%     found while performing these experiments.

% \subsection{Description of CCA.}

%     We will follow here \cite{CortierKeighrenSteel-TACAS-2007} in
%     presentation of the CCA API. This API can be seen a set of rules
%     given below. Following \cite{CortierKeighrenSteel-TACAS-2007}, we
%     present only rules that are crucial from the point of view of key
%     management, and so, from the point of view of safety of the API.

%     The API uses a number of constants (control vectors) that encode
%     types of keys:

%     \begin{center}
%     \begin{tabular}{r@{ -- }p{.36\textwidth}}
%         \data & control vector for data keys, \\
%         \imp  & control vector for import-type key encryption keys, \\
%         \exp  & control vector for export-type key encryption keys, \\
%         \pin  & control vector for pin generation keys, \\
%         \kp   & control vector indicating that a key is only a
%                    part key, not a complete one \\
%     \end{tabular} 
%     \end{center}
%         %
%         %
%     The security module's master key will be denoted by $\km$.
%     This key is the only one stored in the module. All the other keys
%     are stored outside in the form $\e{k}{\km\xor\textit{Type}}$,
%     where \textit{Type} is one of the $\data$, $\imp$, $\exp$ or
%     $\pin$. Such a key is used by the security module only when a key
%     of this type can be used. For example an encrypted key
%     $\e k{\km\xor\data}$ can be used to encrypt/decrypt any general
%     data, while $\e k{\km\xor\imp}$ is used to encrypt other keys.
%     One can observe the different ways key of different types can be
%     used looking at Fig.~\ref{fig:cca}, where
%     the commands of the module are presented. 
%     The commands are given as rules: the left-hand side of a rule is
%     the input to a command and the right-hand side of a rule is the
%     result. \ldots

%     \eqref{cca:enc} and \eqref{cca:dec} commands encrypt/decrypt given
%     plain-text with the supplied data key.  \eqref{cca:exp} converts a
%     working key from being encrypted under the local master key, to
%     being encrypted under the supplied export-type key encryption key.
%     Such a working key can be then imported by some other module using
%     \eqref{cca:imp} command. To do so, however, the same
%     key-inception-key has to be available as an export key in the
%     first module and the import key in the second one. To establish
%     such a shared key one has to use
%     \eqref{cca:first}--\eqref{cca:last} commands. It is supposed to
%     work as follows. A new key encryption key $\kek$ is equal to
%     $k1\xor k2 \xor k3$, where $k1$, $k2$, and $k3$ are known to
%     distinct individuals. The first one performs \eqref{cca:first}
%     with $\typ = \exp$ (or $\typ = \imp$), and sends the result to
%     the second one who performs \eqref{cca:middle} with $x = k1$. In
%     this way he obtains $\e{k1\xor k2}{\km\xor\kp\xor\exp}$ which is
%     to be sent to the third individual who perform \eqref{cca:last}
%     obtaining $\e{k1\xor k2\xor k3}{\km\xor\exp}$.

%     \eqref{cca:transl} translates a key from encryption under one
%     key-encryption-key (of import type) to encryption under another one
%     (of export type). Finally, \eqref{cca:gen} can be used to obtain a
%     randomly generated key of a desired type.

%     \subsection{Known Attacks}

%     \subsubsection*{Bonds Attack.}
%     Do not use key conjuring technique. After the attack the intruder
%     is able to obtain PIN for each account number by invoking an
%     command of the module \eqref{cca:enc}.
    
%     \subsubsection*{IBM Attack.}
%     Key conjuring technique is used. After the attack the intruder
%     posesses the pin-derivation key and so he is able to obtain the
%     PIN for each account number without using the module.

%     \subsection{Analyzing of IBM Recommendations}

%     In response to the published attacks, IBM released a set of
%     recommendations intended to prevent it. As we mentioned, these
%     recommendation were analyzed in [?]. We used our tool to reprove
%     these results.

%     \paragraph*{Recommendation 1} 

%     The discovered attacks exploit some weaknesses in the process of
%     importing keys to the module in three parts. 
%     The first recommendation is to use some public-key technique
%     instead of Key-Part-Import. However, as it is shown in [...], it
%     is not enough to ensure safety of the API. The further means
%     (access control) is needed to prevent attacks. This
%     corresponds to the cases denoted here by 1A and 1B. As these cases are
%     $\xor$-linear, we were able to apply our tool directly, without
%     any modifications. Results are given in Fig.~\ref{exp}.
%     As one can see, the performance is good.

%     We note here again that according to this recommendation, public
%     key encryption (and pairing) should be used. These primitives are
%     not handled by the tool presented in [?] (where some changes in
%     the protocol were made before the protocol was analyzed); they are
%     however, modeled directly by our tool.

%     \paragraph*{Recommendation 2} 

%     Recommendation 2 enforces using access controls to  ensure that no
%     single role is able to mount the attack.
%     We analyzed exactly the same subsets of commands as are analyzed
%     in [...]. This corresponds to the cases denoted here by 2B, 2C
%     and 2E. 
    
%     In these cases non $\xor$-linear rules occur. Hence, our tool
%     could not be applied directly.  However, we were able to obtain
%     equivalent, $\xor$-linear versions, by applying two
%     transformations to each set of horn-clauses to be analyzed: First
%     transformation was one-step \emph{unfolding} [?]. In the second step
%     we applied some simplifications to the rules obtained by unfolding
%     in the first step.  Applying these two steps we were able to get
%     rid of rules which are not $\xor$-linear. Then we could apply our
%     tool. For these cases performance was significantly worse, than
%     previously, but still quite acceptable (one minute in the worst
%     case).

%     % \subsection{A new Attack on CCA\label{sect:attack}} 
%     % In order to present the discovered attack, we need to describe the
%     % CCA API more closely. We will also briefly discussed attack
%     % previously known.



\subsubsection*{Our Attack.}\label{sect:attack}

As we noted before, our tool found an attack
which---according to our knowledge---has not been
discovered before.  This attack uses the same assumptions
as Bond's attack does about the role played by the intruder
and about its knowledge. As in the IBM attack, we use the
fact that $0$ is the default value for $\data$.
  
Our attack does not use key conjuring, and hence, is easier
to carry out than the IBM attack. . As a result of the
attack, the intruder obtains a pin derivation key in clear
(like in the IBM attack).

\medskip In the attack we assume that a new
key-encryption-key $\kek$ needs to be imported, using the
three-part key import commands
\eqref{cca:first}--\eqref{cca:last}, which means that $\kek
= k1\xor k2\xor k3$, where $k1$, $k2$, $k3$ are the shares
known by three different individuals.
  
The key $\kek$ is then used to import a new pin-derivation
key $\pdk$ to the security module, in the form
\begin{equation}\label{pdk}
       \e{\pdk}{\kek\xor\pin}.
\end{equation}
        % 
We assume that this message can be seen by the attacker and
that the attacker is the third participant
of the process of importing $\kek$. In particular, the
attacker can perform \eqref{cca:last}, knows the value $k3$, and obtains the
message
\begin{equation}\label{kp2}
        \e{k1\xor k2}{\km\xor\kp\xor\imp}.
\end{equation}

Now we describe the steps of the attack.  After the
intruder receives \eqref{kp2}, he uses \eqref{cca:last}
with $k3\xor\pin$ instead of $k3$. In this way he obtains
\begin{equation}\tag{A1}\label{at1}
        \e{\kek \xor \pin}{\km\xor\imp}
\end{equation}
He uses the same command again, this time with
$k3\xor\pin\xor\exp$, obtaining:
\begin{equation}\tag{A2}\label{at2}
        \e{\kek \xor \pin \xor \exp}{\km\xor\imp}
<<<<<<< .mine
    \end{equation}

    Next, when $\pdk$ is imported and thus when the intruder can see
    \eqref{pdk}, he uses \eqref{cca:imp} twice: first time for
    \eqref{at1} and \eqref{pdk} with $\typ = \data = 0$, obtaining
    \begin{equation}\tag{A3}\label{at3}
        \e{\pdk}{\km\xor\data}
    \end{equation}
    and second time for \eqref{at2} i \eqref{pdk} with $\typ = \exp$,
    obtaining
    \begin{equation}\tag{A4}\label{at4}
        \e{\pdk}{\km\xor\exp}
    \end{equation}
    Now, using \eqref{cca:exp} for
    \eqref{at3} and \eqref{at4} with $\typ = \data = 0$, he obtains
    \begin{equation}\tag{A5}
=======
\end{equation}
Next, the intruder uses \eqref{cca:imp} twice: The first time with
input \eqref{at1}, \eqref{pdk}, and $\typ = \data = 0$,
resulting in the message
\begin{equation}\tag{A3}\label{at3}
        \e{\pdk}{\km\xor\data}.
\end{equation}
The second time with input \eqref{at2}, \eqref{pdk},
and $\typ =
\exp$, resulting in the message
\begin{equation}\tag{A4}\label{at4}
        \e{\pdk}{\km\xor\exp}.
\end{equation}
Now, using \eqref{cca:exp} with input \eqref{at3},
\eqref{at4}, and $\typ = \data = 0$, the attacker obtains
\begin{equation}\tag{A5}\label{at5}
>>>>>>> .r110
        \e{\pdk}{\pdk\xor\data} = \e\pdk\pdk.
<<<<<<< .mine
    \end{equation}
    From this and \eqref{at3}, using \eqref{cca:dec}, the intruder
    can obtain the clear value of $\pdk$ which can be used to
    obtain the PIN for any account number.
=======
\end{equation}
Finally, using \eqref{cca:dec} with input \eqref{at5} and
\eqref{at3}, the attacker obtains the clear value of
$\pdk$, which can be used to obtain the PIN for any account
number.
>>>>>>> .r110


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "xorpro-rep"
%%% End: 

